Extremum Seeking for Controlled Vibrational Stabilization of Second Order Mechanical Systems

This paper presents a novel extremum seeking control (ESC) approach for the vibrational stabilization of a class of mechanical systems (e.g., systems characterized by equations of motion resulting from Newton second law or Euler-Lagrange mechanics). Inspired by flapping insects mechanics, the proposed ESC approach is operable by only one perturbation signal and can admit generalized forces that are quadratic in velocities. We test our ESC, and compare it against approaches from literature, on some classical mechanical systems (e.g., mass-spring and an inverted pendulum systems). We also provide a novel, first-of-its-kind, application of the introduced ESC by achieving a 1D model-free source-seeking of a flapping system.

==> PSMacros.tex <==
% Packages and macros go here:
 \usepackage{etex}
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf} 
\usepackage{enumerate} 
 \usepackage{amsmath}  
 \usepackage{subfig,bbm,enumerate,multirow,framed,blkarray}   


\usepackage{verbatim,tcolorbox}
  \usepackage{tikz}
\usetikzlibrary{shapes,arrows}
\usetikzlibrary{positioning}  
\usepackage{pstricks-add} 
 \usepackage{wrapfig}
 \usepackage{pgfplots}
  
\usepackage{color}
\usepackage{savesym}
%\savesymbol{AND} 
\usepackage[noend]{algpseudocode} 
%\usepackage{algorithm} 
%\usepackage{algorithmic}  
%\usepackage[algo2e]{algorithm2e} 
% \usepackage{algpseudocode} 
% \usepackage{algorithm2e} 
 \usepackage{graphicx}          % Include this line if your 
                               % document contains figures,
%\usepackage[dvips]{epsfig}    % or this line, depending on which
                               % you prefer.

%% algorithm commands:

%\algnewcommand\And{\textbf{and }}
%\algnewcommand\Or{\textbf{or }}
%\algnewcommand{\algorithmicgoto}{\textbf{go to}}%
%\algnewcommand{\Goto}[1]{\algorithmicgoto~\ref{#1}}%



%%COMMANDS AND STYLES: 
 \DeclareMathOperator*{\sign}{sign}  
\DeclareMathOperator*{\fsign}{fsign} 
 \DeclareMathOperator*{\argmax}{argmax} 
 \DeclareMathOperator*{\argmin}{argmin} 
 
% \theoremstyle{definition}  
\newtheorem{theorem}{Theorem}[section] 
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{definition}[theorem]{Definition} 
\newtheorem{remark}[theorem]{Remark}
\newtheorem{remarks}[theorem]{Remarks}
\newtheorem{assumption}[theorem]{Assumption} 
\newtheorem{example}[theorem]{Example} 
  

\newcommand{\solnvi}{\text{SOL}(K,\mathbf{F})}
%\newcommand{\solnncp}{\text{SOL}_{\text{NCP}}(\mathbf{F})}
%\newcommand{\solnlcp}{\text{SOL}_{\text{LCP}}(\mathbf{y},\mathbf{M})}
%\newcommand{\solnlelcp}{\text{SOL}_{\text{LeLCP}}(\mathbf{y},\mathbf{M})}
\newcommand{\solnncp}{{\text{NCP}}(\mathbf{F})}
\newcommand{\solnlcp}{{\text{LCP}}(\mathbf{y},\mathbf{M})}
\newcommand{\solnlelcp}{{\text{LeLCP}}(\mathbf{y},\mathbf{M})}

\newcommand{\anot}{\aaa_0}
\newcommand{\bnot}{\bbb_0}
\newcommand{\psib}{\pmb{\Psi}} 
\newcommand{\xib}{\pmb{\Xi}} 
%%%%%
\newcommand{\conv}{\text{conv}}
\newcommand{\plen}{\text{plen}}
 \newcommand{\fdir}{\mathbf{fdir}}
\newcommand{\qpstrong}{\mathcal{A}^+_{\text{QP}}}	
\newcommand{\qpweak}{\mathcal{A}^0_{\text{QP}}}
\newcommand{\qpinact}{\mathcal{A}^-_{\text{QP}}}
\newcommand{\qpact}{\mathcal{A}_{\text{QP}}}  
\newcommand{\cone}{P}  
\newcommand{\qp}{\text{QP}}
\newcommand{\lp}{\text{LP}}	 
   \newcommand{\strong}{\mathcal{A}^+}	
\newcommand{\weak}{\mathcal{A}^0}
\newcommand{\weakcrit}{\beta_{\text{crit}}}
\newcommand{\inact}{\mathcal{A}^-}
\newcommand{\act}{\mathcal{A}} 
\newcommand{\pset}{\mathcal{P}}
\newcommand{\iset}{\mathcal{I}}
\newcommand{\jset}{\mathcal{J}}
\newcommand{\nset}{\mathcal{N}}
\newcommand{\gset}{\mathcal{G}}
\newcommand{\sset}{\mathcal{S}}
\newcommand{\hset}{\mathcal{H}} 
	\algnewcommand\And{\textbf{and }}
	\algnewcommand\Or{\textbf{or }}
\newcommand{\pnot}{\pp_0}
\newcommand{\xnot}{\x_0}
\newcommand{\unot}{\uu_0}
\newcommand{\munot}{\mumu_0}
\newcommand{\etanot}{\etaeta_0} 
\newcommand{\rhonot}{\rhorho_0} 
\newcommand{\gamnot}{\gamgam_0} 
\newcommand{\gammanot}{\gamgam_0} 
\newcommand{\lambdanot}{\lambdalambda_0}
\newcommand{\dnot}{\dd_0} 
\newcommand{\ynot}{\mathbf{y}_0}
\newcommand{\znot}{\mathbf{z}_0} 
\newcommand{\vnot}{\mathbf{v}_0}

\newcommand{\minmin}{\pmb{\text{min}}}
\newcommand{\maxmax}{\pmb{\text{max}}}
\newcommand{\opt}{\pmb{\Phi}}
\newcommand{\mumu}{\pmb{\mu}}
\newcommand{\btheta}{\pmb{\theta}}
\newcommand{\nunu}{\pmb{\nu}}
\newcommand{\lambdalambda}{\pmb{\lambda}}
\newcommand{\deltadelta}{\pmb{\delta}}
\newcommand{\sx}{\widetilde{\pmb{x}}}
\newcommand{\smu}{\widetilde{\pmb{\mu}}}
\newcommand{\capmu}{\mathbf{U}}
\newcommand{\caplambda}{\mathbf{W}}
\newcommand{\lmin}{\mathbf{Lmin}}
\newcommand{\slmmin}{\mathbf{SLMmin}}
\newcommand{\lmmin}{\mathbf{LMmin}}
\newcommand{\lshiftmin}{\mathbf{SLmin}}
\newcommand{\lmax}{\mathbf{Lmax}}
\newcommand{\slmmax}{\mathbf{SLMmax}}
\newcommand{\lmmax}{\mathbf{LMmax}}
\newcommand{\lshiftmax}{\mathbf{SLmax}} 
\newcommand{\shift}{\mathbf{shift}}
\newcommand{\lmid}{\mathbf{Lmid}}
\newcommand{\lshiftmid}{\mathbf{SLmid}}
\newcommand{\coord}{\mathbf{e}} 
\newcommand{\E}{\mathbf{E}} 
\newcommand{\capw}{\mathbf{W}}
\newcommand{\caps}{\mathbf{S}}
\newcommand{\phimin}{\pmb{\Phi}_{\min}}
\newcommand{\phincp}{\pmb{\Phi}_{\text{NCP}}}
\newcommand{\psincp}{\pmb{\psi}_{\text{NCP}}}
\newcommand{\n}{\mathbf{n}}
\newcommand{\ximp}{\widetilde{\mathbf{x}}}
\newcommand{\zimp}{\widetilde{\mathbf{z}}}
\newcommand{\muimp}{\widetilde{\pmb{\mu}}}
\newcommand{\lambdaimp}{\widetilde{\pmb{\lambda}}}
\newcommand{\etaimp}{\widetilde{\pmb{\eta}}} 
%%%%%%%%%%%%%
\newcommand{\setmapsto}{\rvert\!\!\!\rightrightarrows}
\newcommand{\real}{\mathbb R}
\newcommand{\posint}{\mathbb{N}} 
\newcommand{\eps}{\epsilon}    
\newcommand{\tint}{[t_0,t_f]}
\newcommand{\fbar}{\hat{\mathbf{f}}_t}
\newcommand{\Fbar}{\hat{\mathbf{F}}_t} 
\newcommand{\gbar}{\hat{\mathbf{g}}_t}
\newcommand{\zx}{\pmb{\eta}_x}  
\newcommand{\zy}{\pmb{\eta}_y}
\newcommand{\zp}{\pmb{\eta}_p}
\newcommand{\etaxdot}{\pmb{\eta}_{\dot{x}}} 
\newcommand{\etaz}{\pmb{\eta}_z}  
\newcommand{\etazdot}{\pmb{\eta}_{\dot{z}}} 
\newcommand{\etaeta}{\pmb{\eta}}    
\newcommand{\rhorho}{\pmb{\rho}}  
\newcommand{\gamgam}{\pmb{\gamma}}
\newcommand{\zdot}{\mathbf{\dot{z}}}
\newcommand{\zz}{\mathbf{z}}
\newcommand{\w}{\mathbf{w}} 
\newcommand{\aaa}{\mathbf{a}}
\newcommand{\bbb}{\mathbf{b}}
\newcommand{\uu}{\mathbf{u}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\qq}{\mathbf{q}}
\newcommand{\zxdot}{\mathbf{z_{\dot{x}}}}   
\newcommand{\dx}{\mathbf{d_x}}   
\newcommand{\dy}{\mathbf{d_y}}   
\newcommand{\f}{\mathbf{f}}
\newcommand{\TT}{\mathbf{T}}
\newcommand{\kk}{\mathbf{k}}
\newcommand{\mm}{\mathbf{m}}
\newcommand{\F}{\mathbf{F}}
\newcommand{\phiphi}{\pmb{\phi}} 
\newcommand{\GammaGamma}{\pmb{\Gamma}} 
\newcommand{\XiXi}{\pmb{\Xi}} 
\newcommand{\g}{\mathbf{g}}
\newcommand{\dd}{\mathbf{d}}
\newcommand{\h}{\mathbf{h}}
\newcommand{\x}{\mathbf{x}} 
\newcommand{\widex}{\mathbf{\widetilde{x}}}
\newcommand{\widey}{\mathbf{\widetilde{y}}}
\newcommand{\wider}{\mathbf{\widetilde{r}}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\M}{\mathbf{M}}
\newcommand{\I}{\mathbf{I}}
\newcommand{\K}{\mathbf{K}}
\newcommand{\C}{\mathbf{C}}
\newcommand{\II}{\mathbf{I}}
\newcommand{\PP}{\mathbf{P}}
\newcommand{\HH}{\mathbf{H}}
\newcommand{\GG}{\mathbf{G}}
\newcommand{\A}{\mathbf{A}}
\newcommand{\D}{\mathbf{D}}
\newcommand{\B}{\mathbf{B}}
\newcommand{\m}{\mathbf{m}}
\newcommand{\N}{\mathbf{N}}
\newcommand{\LL}{\mathbf{L}}
\newcommand{\Q}{\mathbf{Q}}
\newcommand{\biggamma}{\mathbf{\Gamma}} 
\newcommand{\rr}{\mathbf{r}}
\newcommand{\capx}{\mathbf{X}}
\newcommand{\capQ}{\mathbf{Q}}
\newcommand{\capE}{\mathbf{E''_q}}
\newcommand{\capVref}{\mathbf{V_{ref}}}
\newcommand{\capw}{\mathbf{W}}
\newcommand{\capr}{\mathbf{R}}
\newcommand{\capf}{\mathbf{F}}
\newcommand{\capp}{\mathbf{P}}
\newcommand{\capu}{\mathbf{U}}
\newcommand{\capv}{\mathbf{V}}
\newcommand{\capz}{\mathbf{Z}}
\newcommand{\capzdot}{\mathbf{\dot{Z}}}
\newcommand{\capy}{\mathbf{Y}}
\newcommand{\capxdot}{\dot{\mathbf{X}}} 
\newcommand{\cc}{\mathbf{c}}
\newcommand{\cnot}{\cc_0}
\newcommand{\pp}{\mathbf{p}} 
\newcommand{\dee}{\mathbf{d}}
\newcommand{\zero}{\mathbf{0}}
\newcommand{\one}{\mathbf{1}}
\newcommand{\batx}{\mathbf{\hat{x}}}
\newcommand{\xt}{\mathbf{x}_t}
\newcommand{\yt}{\mathbf{y}_t}
\newcommand{\rt}{\mathbf{r}_t}
\newcommand{\ex}{\mathbf{e_x}}
\newcommand{\ey}{\mathbf{e_y}}
\newcommand{\ef}{\mathbf{e_f}}
\newcommand{\eg}{\mathbf{e_g}}
\newcommand{\Jf}{\mathbf{Jf}}
\newcommand{\J}{\mathbf{J}}
\newcommand{\JLf}{\mathbf{J}_{\text{L}} \mathbf{f}}
\newcommand{\xset}{\mathcal{X}}
\newcommand{\zset}{\mathcal{Z}} 
\newcommand{\LS}{LS} 
\newcommand{\reg}{\mathcal{Z}^{\text{R}}}
\newcommand{\irreg}{\text{IRREGSOL}}
\newcommand{\bomega}{\pmb{\omega}}  
 
\algnewcommand{\algorithmicgoto}{\textbf{go to}}%
\algnewcommand{\Goto}[1]{\algorithmicgoto~\ref{#1}}%
 
\newenvironment{bsmallmatrix}{\left[\begin{smallmatrix}}{\end{smallmatrix}\right]}

